The plaid model and outer billiards on kites

This paper is the third in a series which explores a combinatorial method for generating lattice polygons in the plane. I call this method the plaid model. In this paper I prove the main result I had been aiming for since the beginning, which is to show that there is a coarse isomorphism between the plaid model and the so-called arithmetic graph for outer billiards on kites. The content of the theorem is that the plaid model predicts the symbolic dynamics of the outer billiards orbits, up to an error of one unit. This result combines with the work in the other papers to give a second proof that outer billiards has unbounded orbits for every irrational kite. So far, these are the only known polygonal examples with this property.

==> 14tut.tex <==
\section{Tutorial}

==> Backup/3poly.tex <==
\section{Polygon Families}

\subsection{Nice Families}
\label{poly}

In this chapter we prove a result which is similar
in spirit to Lemma \ref{vertical1} but more general.
This result will allow us to compare the diverse
families of polygons, such as those shown in
Figure 1.

Let $F$ be a union of pairwise disjoint and
embedded polygons in the plane.  We say that
$F$ {\it sits poorly \/} with respect to a
square $S$ if some horizontal line which
 intersects two components of $F \cap S$.
Figure 3.1 shows some examples of this.

\begin{center}
\resizebox{!}{1.7in}{\includegraphics{Pix/poor.eps}}
\newline
{\bf Figure 3.1:\/} polygons sitting poorly
with respect to squares
\end{center}

If $F$ does not sit poorly with respect to $S$,
we say that $F$ {\it sits nicely\/} with respect
to $S$. We call $F$ {\it nice\/} if \begin{enumerate}
\item $F$ sits
nicely with respect to every integer unit square.
\item $F$ does not cross an integer vertical line at a
vertex of an integer square.
\item $F$ crosses each unit vertical edge at most once.
\end{enumerate}

There are some situations where $F$ will contain a
point on a unit vertical edge, but not cross there.
We do not count these as intersections. 

Let $L$ be a vertical line segment whose endpoints
have integer coordinates.  Note that $L$ is
a subset of one of the $\cal V$ lines, and also
$L$ is a finite union of vertical unit segments.
By construction, $F \cap L$ is a finite union
of points, and there is at most one point in
each unit vertical segment of $L$.  We let
$F_L$ denote the union of the center points of the
unit vertical segments of $L$ which contain points of
$F \cap L$.  There is a natural bijection between
$F \cap L$ and $F_L$ which moves points by less
than $1/2$ units.  The set $F_L$ is just a tidier
version of $F \cap L$.

\subsection{Straigntening a Nice Family}

Say that a {\it connector\/}
in a unit integer square is
a line segment which connects
the midpoints of a pair of edges of the
square.  This is as in \S \ref{PETS}.
 Say that $A$ is {\it straight\/}
if the intersection of $A$ with each
unit integer square is either the
emptyset or a connector.
The family of plaid polygons for any
parameter is straight.

\begin{lemma}
\label{straight}
There is a straight family $A'$ with the
following properties:
\begin{itemize}
\item $A' \cap L=A_L$ for every $\cal V$ line $L$.
\item There is a homeomorphism which
maps the components of $A \cap X$
to the components of $A' \cap X$
extending the bijection from $A \cap L$ to $A_L$
on every $\cal V$ line $L$.
\item Two components which correspond {\it via\/}
the homeomorphism are $\sqrt 2$-quasi-isomorphic.
\end{itemize}
\end{lemma}

\startproof
Basically we just straighten $A$ out and
get $A'$.  Let $S$ be some square of $X$.
If $S$ is disjoint from $A_1 \cup A_2$ then
for $A'$ we leave $S$ as an empty square.
Suppose that $A_1$ intersects (say) the left
side of $S$ in a point $a_1$.  Let $\alpha_1$ be the component
of $A \cap X$ which has $a_1$ as an endpoint.
If $\alpha_1$ leaves $S$ and returns, then we
would get a contradiction to the niceness
property.  So, $\alpha_1$ remains in $S$ until
it exits a side.   For $A'$ we simply put
in the tile which connects the midpoints
of the two sides containing the endpoints
of $\alpha_1$.

We want to make sure that our definition
is consistent.  Suppose that there was
a second point $a_2 \in A_2$ in the
right hand side of $S$.  Let $\alpha_2$ be
the component of $X \cap A$ which has
$a_2$ as an endpoint.  If $\alpha_1 \not = \alpha_2$
then we would contradict the niceness property.
Hence, $\alpha_1=\alpha_2$.  So, starting
with either $a_1$ or $a_2$ we would produce
the same tile.  This argument shows that
that the definition of $A'$ is consistent.

By construction, consecutive tiles match
up along their tops and bottoms. 
Since our modification is done locally,
square by square, corresponding components
can be parametrized so that they stay with
$\sqrt 2$ units of each other.  Here
$\sqrt 2$ is the diameter of a unit integer
square.
\endproof


\subsection{Nice Pairs}

Suppose that $A$ and $B$ are two nice families.
Let $L$ be an integer vertical line segment, as above.
We write $A_L \approx B_L$ if these two
sets have the same number of points and if the
order-preserving bijection between the points
moves each point by at most $1$ unit.  

Let $L_1$ and $L_2$ be two consecutive
vertical lines.
Figure 3.2 shows a configuration of points
contained in the union 
$$A_{L_1} \cup A_{L_2} \cup B_{L_1} \cup B_{L_2}.$$
We call this configuration, and also
its mirror image, a {\it switch\/}.
\begin{center}
\resizebox{!}{1.5in}{\includegraphics{Pix/switch.eps}}
\newline
{\bf Figure 3.2:\/} The switch configurations.
\end{center}
The black dots are $A$-points and the white dots are
$B$-points.  On each line $L$ the
bijection between $A_L$ and $B_L$
pairs up the black and white points on that line.

We say that the pair $(A,B)$ is {\it nice\/} if
$A$ and $B$ are nice separately, and there are
no switches.

\subsection{The Main Result}

Let $X$ be a rectangle whose sides are parallel
to the coordinate axes and whose vertices have
integer coordinates.  Let $X_H$ denote the union
of the top and bottom edge of $X$.  Here is our
main result.

\begin{lemma}[Vertical]
Let $(A,B)$ be a nice pair
with both $A$ and $B$ straight.
Suppose 
 $A \cap X_H=B \cap X_H = \emptyset$
and $A_L \approx B_L$ for all integer vertical
line segments $L$ of $X$.  Then there is a
homeomorphism from $A \cap X$ to $B \cap X$
such that corresponding components are
$1$-quasi-isomorphic.
\end{lemma}

Combining Lemma \ref{straight} and the
Vertical Lemma, we get the following corollary.


\begin{corollary}
Let $(A,B)$ be a nice pair.
Suppose 
 $A \cap X_H=B \cap X_H = \emptyset$
and $A_L \approx B_L$ for all integer vertical
line segments $L$ of $X$.  Then there is a
homeomorphism from $A \cap X$ to $B \cap X$
such that corresponding components are
$(1+2\sqrt 2)$-quasi-isomorphic.  If
one of the families
is straight, then one can take the
constant to be $1+\sqrt 2$.
\end{corollary}


We will prove the Vertical Lemma through a series
of smaller lemmas. First of all, 
we reduce to a special case.
We can write $X=X_1 \cup ... \cup X_k$, where each
$X_j$ is a rectangle which is $1$ unit thick.
It suffices to prove our result for each
rectangle $X_j$ separately, because then
the corresponding homeomorphisms
$h_1,...,h_k$ piece together across the
vertical boundaries to produce one global
homeomorphism.  The quasi-isomorphism
constants do not increase when we do this.
So, it suffices to
consider the case where the width of $X$ is $1$
unit.

Let $X_1$ and $X_2$ denote the left
and right edges of $X$.  Let
\begin{equation}
A_j=A \cap X_j, \hskip 40 pt
B_j=B \cap X_j.
\end{equation}
For $j=1,2$ we have a bijection from
$A_j$ to $B_j$.  We want to extend
this bijection to a homeomorphism
from $X \cap A$ to $X \cap B$.

There are two kinds of components of
$X \cap A$, those which have their
endpoints on different sides and those
which do not. We call the first kind
of component a {\it crosser\/} and
the second kind of component a
{\it noncrosser\/}.   Because $A$ is
clean, any noncrossing component connects
adjacent points on the boundary.

The rule for crossers is more complicated.
Let $a \in A_1$.  Let $a'$ be the point
on $X_2$ directly across from $a$.  Then
the component of $X \cap A$ which contains
$a$, provided that it is a crosser,
has one of three possible endpoints
on $X_2$:
\begin{itemize}
\item The point $a'$.  This happens if and only
if $a' \in A_2$.
\item The nearest point of $A_2$ above $a'$.
\item The nearest point of $A_2$ below $a'$.
\end{itemize}
For later reference, we call this
the {\it trichotomy rule\/}.
All these considerations apply to $B$ as well.

\begin{lemma}
The Vertical Lemma is true provided that
the bijection on the boundary extends to
the crossers.
\end{lemma}

\startproof
Suppose we have a
bijection between the crossers of $A$ and
the crossers of $B$ which extends the
bijection on the boundary.  Then the
consecutive points property guarantees that
the non-crossers form the same pattern
for both $A$ and $B$. This allows us to
extend the bijection to the non-crossers.

It remains to show that corresponding
components are $1$-quasi-isomorphic.
Let $\alpha$ and $\beta$ be two corresponding
components.  The corresponding endpoints of these
components differ from each other by at
most $1$ unit.  If the minimum separation
between the endpoints of $\alpha$ and 
$\beta$ is at least $4$ then both 
$\alpha$ and $\beta$ look like the
paths shown in Figure 3.3 or
the mirror images of these.

\begin{center}
\resizebox{!}{2in}{\includegraphics{Pix/comp.eps}}
\newline
{\bf Figure 3.3:\/} Two kinds of components
\end{center}

The length of the vertical part can
change by at most $2$ units when we
pass from $\alpha$ to $\beta$.
In this situation it is easy to see that
the two components are $1$-quasi-isomorphic.
There are only a small number of possibilities
when the minimum separation is less than $3$,
and a case by case examination of these
reveals that this case works out as well.
\endproof

Now we will show that our bijection extends to the
crossers.   We label the points of $A_1$ as
$a_{1,1},...,a_{1,N}$, starting from the bottom.
We label the points of the sets $A_2,B_1,B_2$
similarly.  In general, we way that one point
lies above another if it has a larger $y$-coordinate.
Similarly, a point lies above an interval if
the point lies above the top endpoint of the
interval.

Suppose that we have an $A$-crosser $\alpha$
that connects $a_{1,m}$ to $a_{2,n}$.  We want
to see that there is a $B$-crosser that
connects $b_{1,m}$ to $b_{2,n}$.   Let
$\beta$ be the component of $X \cap B$ which
contains $b_{1,m}$.  There are two cases
to consider.
\newline
\newline
{\bf Case 1:\/} 
Suppose that $\beta$ is a crosser.
Let $a_{1,m'}$ be as in the trichotomy rule.
The trichotomy rule implies that the segment
bounded by $a_{2,n-1}$ and $a_{2,n+1}$ contains
$a_{1,m}'$ in its interior.  More precisely,
$a_{1,m}'$ is at least $1$ unit from the
boundary of this segment.  Since there are
no switches, 
the segment bounded by $b_{2,n-1}$ and $b_{2,n+1}$
contains $b_{1,m}'$.
But then
$\beta$ connects $b_{1,m}$ to one of the
three points $b_{2,k}$ for $k \in \{n-1,n,n+1\}$.

Parity considerations rule out two of the
possibilities.  If $\beta$ connects
$b_{1,m}$ to $b_{2,n \pm 1}$ then 
$\beta$ divides the remaining points
of $B_1 \cup B_2$ into two halves, each
containing an odd number of points. But then
these points cannot be paired up by the
arcs of $X \cap B$.  So, 
$\beta$ connecta $b_{1,m}$ to $b_{2,n}$,
as desired.
\newline
\newline
{\bf Case 2:\/} Suppose that $\beta$ is a non-crosser.
Then $\beta$ connects $b_{1,m}$ to $b_{1,m\pm 1}$.
Without loss of generality, consider the case when
$\beta$ connects $b_{1,m}$ to $b_{1,m+1}$.
Since $B$ is a
clean family, there can be no point of $B_2$
in the interval $I$ bounded by $b_{1,m}'$ and
$b_{1,m+1}'$.  In particular,
$b_{2,n}$ either lies above $I$ or below $I$.
We claim that $b_{2,n}$ lies above $I$.   
Assume this claim for the moment.
Since there are no switches,
$a_{2,n}$ is at the same height as
$a_{1,m+1}$ or above it.  But this
is impossible in a clean family.
Every point of $A_1-\{a_{1,m}\}$
either lies below $a_{1,m}$ or
above $b_{2,n}$.

Now we deal with our claim.
The same analysis as in Case 1 shows that
$b_{1,m'}$ lies in the interval bounded
by $b_{2,n-1}$ and $b_{2,n+1}$.  Therefore,
$b_{2,n-1}$ lies below $I$ and
$b_{2,n+1}$ lies above $I$.
Let $A_1^k$ denote the points of $A_1$ above 
or equal to $a_{1,k}$.
Likewise define $A_{2,k}$, etc.
Since $\alpha$ is a connector, 
$A_1^{m+1} \cup A_2^{n+1}$ has an even number $E$ of points.
Note that $B_1^{m+1} \cup B_2^{n+1}$ has $E$ points
as well.
Since $B$ is a straight family, the
points of $B_1 \cup B_2$ above $I$ must be
paired together.  If $b_{2,n}$ lies below $I$,
then $B_1^{m+2} \cup B_2^{n+1}$ has an
even number of points.  But this is false,
because $B_1^{m+2} \cup B_2^{n+1}$ has $E-1$ points.
This establishes the claim.
\newline

Now we have shown that our bijection extends to
crossers. As we have already established, this suffices
to prove the Vertical Lemma.


\end{document}
\newpage

==> Backup/5geom.tex <==
\section{Geometry of the Classifying Map}

\subsection{Pulling Back the Maps}

Now we will take steps to bring the
arithmetic graph in line with the
plaid model.
Let $T_A$ be the map given in Equation \ref{affine}.
Let 
\begin{equation}
\Theta_A=T_A(\Z^2).
\end{equation}
The set
$\Theta_A$ is an affine lattice, in the sense that
is is the translated image of an ordinary lattice
in $\R^2$.  The ordinary lattice is
\begin{equation}
\label{linearlat}
L\Theta_A=\Theta_A-(0,\widehat \tau).
\end{equation}
We can apply the Master Picture Theorem directly
to $\Theta_A$. We simply replace the map
$f_{\pm}$ with the composition
\begin{equation}
g_{\pm} = f_{\pm} \circ T_A^{-1}.
\end{equation}
and we replace each label $V$ of the partition by
$T_A(V)$.  The partition itself stays the same.

The maps $g_{\pm}$ are locally affine maps and
so we think of them as having $\R^2$ as their domain.
Setting
$(\widehat x,\widehat y)=dT^{-1}(x,y)$. We use
Equation \ref{diffinv} to compute that
\begin{equation}
A\widehat x + \widehat y = x.
\end{equation}
Therefore, there are constant vectors $C_{\pm}$, depending
on $A$, such that
$$
g_{\pm}(x,y)=(x,x,x)+c_{\pm} \hskip 10 pt
{\rm mod\/} \hskip 5 pt \Lambda_A.
$$
In particular, $g_{\pm}$ is constant along
vertical lines.  Because
$g_{\pm}$ is constant along vertical lines,
we have
$$g_{\pm}(0,0)=g_{\pm}(0,\widehat \tau)=
f_{\pm}(0,0)=(-\frac{1}{2},\frac{1}{2},0) \pm (\frac{1}{2},\frac{1}{2},0). 
\hskip 10 pt {\rm mod\/} \hskip 5 pt \Lambda_A.$$
From this we conclude that
\begin{equation}
g_{\pm}(x,y)=\bigg(x-\frac{1}{2},x+\frac{1}{2},x\bigg) 
\pm \bigg(\frac{1}{2},\frac{1}{2},0\bigg) 
\hskip 10 pt {\rm mod\/} \hskip 5 pt \Lambda_A.
\end{equation}
In other words, we get exactly the same formula
as we got for $f_{\pm}$ except that $Ax+y$ is
replaced by $x$.

\subsection{Periodicity}

Let $A=p/q$.
The map $dT^{-1}$ carries $\Theta_A$ to $\Z^2$.
Here is the formula again:
$$
dT^{-1}=
\frac{1}{2A}\left(\matrix{P^2&P\cr P^2+P-PA & -PA}\right).
$$
group of translations generated by the translation
vectors $(0,\omega)$ and $(\omega^2,0)$.

\begin{lemma}
Both
$\Theta_A$ and $T_A(\Gamma_A)$ are invariant under translation by
$(0,\omega)$ and $(\omega^2,0)$.
\end{lemma}

\startproof
We first check this for $\Theta_A$.
It suffices to prove that
$dT^{-1}(0,\omega)$ and  $dT^{-1}(\omega^2,0)$
both belong to $\Z^2$.
Using the fact that $P/A=Q$, we have
$$dT^{-1}(0,\omega)=\frac{1}{2}\left(
\matrix{Q\omega\cr -P\omega}\right)=
\left(\matrix{q \cr -p}\right).$$

$$dT^{-1}(\omega^2,0)=
\frac{1}{2}\left(
\matrix{\omega^2PQ \cr
\omega^2 PQ + \omega^2Q-\omega^2P}\right)=
\left(\matrix{2pq \cr
2pq+q^2 -p^2} \right).$$
Both images are in $\Z^2$.

Now we check the invariants of $T_A(\Gamma_A)$.
The maps $g_{\pm}$ are constant along vertical
lines, so certainly
$g_{\pm}((x,y)+(0,\omega))=g_{\pm}(x,y)$.
It remains to check that
$$g_{\pm}((x,y)+(\omega^2,0))=g_{\pm}(x,y).$$
This is equivalent to the statement that
$(\omega^2,\omega^2,\omega^2) \in \Lambda_A$.
Here $\Lambda_A$ is the lattice in Equation \ref{lattice}.
Let $C_1,C_2,C_3$ be the three columns of this matrix.
We have
$$q\omega C_1=\left(\matrix{\omega^2 \cr 0 \cr 0} \right),
\hskip 30 pt
\omega^2 C_3=\left(\matrix{-\omega^2 \cr -\omega^2\cr \omega^2} \right),$$
$$2pq(C_1+C_2)+q^2(-C_1+C_2)=
\left(\matrix{2pq \cr p\omega \cr 0}\right)+
\left(\matrix{-2pq \cr q\omega \cr 0}\right)=
\left(\matrix{0\cr \omega^2 \cr 0} \right).
$$
Clearly $(\omega^2,\omega^2,\omega^2)$ is the
sum of the vectors we have generated so far.
\endproof

In view of these two results, it suffices to prove the
Quasi-Isomorphism Theorem for the portion of the arithmetic
graph inside the fundamental domain $\Xi$ for the plaid model.
Here $\Xi$ is the union of the blocks
$B_k$ for $k=0,...,(\omega-1)$.   

\subsection{Coincidence Points}
\label{coincidence}

The sets $\Theta_A$ and $\Z^2$ are quite different, but
there are a few points where we can say that they
coincide.  These points will be useful when we try
to make arguments that involve both sets.  For instance
\begin{equation}
(0,\widehat \tau) \subset \Theta_A \cap \Z^2.
\end{equation}
Here $\widehat \tau$ is such that
$2p\widehat \tau = 1$ mod $\omega$.
Here we find a second such point.
Let $\xi \in (0,\omega)$ be such that
\begin{equation}
4p^2 \xi \equiv 1 \hskip 5 pt
{\rm mod\/} \hskip 5 pt \omega.
\end{equation}

\begin{lemma}
$(\xi \omega,0) \in \Theta_A \cap \Z^2$.
\end{lemma}

\startproof
Clearly this point lies in $\Z^2$.  It suffices
to prove that
$T_A^{-1}(\xi \omega,0) \in \Z^2.$
We compute that $T_A^{-1}(\xi \omega,0)=(A_1,A_2+A_3)$, where
$$A_1=\frac{PQ\xi \omega-Q\widehat \tau}{2}, \hskip 30 pt
A_2\frac{PQ\xi \omega+P\widehat \tau}{2}, \hskip 30 pt
A_3=\frac{Q\xi\omega-P\xi\omega}{2}.$$
We will show that each of these expressions is an integer.
\begin{equation}
\label{A1}
A_1=q\bigg(\frac{2p\xi-\widehat \tau}{\omega}\bigg).
\end{equation}
Since 
$$4p^2 \xi \equiv 2p\widehat \tau \hskip 5 pt
{\rm mod\/} \hskip 5 pt \omega,$$
and since $2p$ is relatively prime to $\omega$, we
see that $2p\xi \equiv \widehat \tau$ mod $\omega$.
Hence, the expression inside the parentheses in Equation
\ref{A1} is an integer. Hence $A_1 \in \Z$.
Next, we have
$$A_2-A_1=\frac{(P+Q)\widehat \tau}{2}=\widehat \tau \in \Z.$$
Hence $A_2 \in \Z$.
Finally,
$$A_3=q\xi-p\xi \in \Z.$$
This completes the proof.
\endproof

\subsection{The Reconstruction Formula}




Let $A=p/q \in (0,1)$.
In this section we discuss the geometry of the maps
$g_{\pm}: \Theta_A \to R_A$ in more detail.
For convenience, we repeat the definition
of the lattice $\Lambda_A$:
\begin{equation}
\Lambda_A=\left[\matrix{
1+A & 1-A & -1 \cr
0 & 1+A & -1 \cr
0 & 0 & 1}\right] \Z^3
\end{equation}


Note that $g_{\pm}$ depends on $A$, but our
notation suppresses this.
We will explain how the maps $g_{\pm}$ actually detect
the geometry of the lattice $\Theta_A$.  

Given a point $\xi \in \Theta_A$, let
$[\xi] \in \R^2/\Z^2$ denote the
equivalence class of $\xi$.
We now explain how we can use the map
$g_+$ to determine $[\xi]$.  Of course,
we could also use $g_-$, with slightly
different formulas.

We introduce the affine maps $L_1,L_2: \R^3 \to \R$:
\begin{equation}
L_1(x,y,z)=z, \hskip 30 pt
L_2(x,y,z)=\frac{y-Az-1}{1+A}.
\end{equation}

Let $L_j'$ be the linear part of $L_j$.  Checking
on the obvious basis for $\Lambda_A$, we see
that $L_j'(\Lambda_A) \subset \Z$.  Therefore
$L_1$ and $L_2$ both give well defined
maps from $R_A=\R^3/\Lambda_A$ into $\R/\Z$.
Hence, we have a locally affine map
\begin{equation}
\Phi: R_A \to \R^2/\Z^2, \hskip 30 pt
\Phi=[(L_1,L_2)].
\end{equation}


The goal of this section is to establish
the following equation
\begin{equation}
\label{reconstruct}
\Phi \circ g_+(\xi)=[\xi].
\end{equation}
We call this equation the
Reconstruction Formula.
Equation \ref{reconstruct}
allows us to get control over how the
arithmetic graph sits with respect to
$\Z^2$, and we will use it in
our proof that
the arithmetic graph is
a nice family of polygons.

We found Equation
\ref{reconstruct} by trial and error,
and in this section
we will give a completely computational
proof.  We discovered the formula by
thinking about the results discussed
later on in this chapter.


Recall that $\Theta_A=T_A(\Z^2)$.
Our first result is kind of a sanity
check for the overall equation.

\begin{lemma}
\label{easy}
Equation \ref{reconstruct} holds 
at the lattice point $\xi=T_A(0,0)$.
\end{lemma}

\startproof
By construction $\xi=(0,\widehat \tau) \in \Z^2$. Hence
$[\xi]=(0,0)$.  On the other hand
$g_+(\xi)=f_+(0,\widehat \tau)=(0,1,0)$ and
so $\Phi \circ g_+(\xi)=[(0,0)]$ as well.
\endproof

\begin{lemma}
\label{explicit}
Equation \ref{reconstruct} holds
for $A=1/2$ and also for
$$A=\frac{1}{2}+\frac{2k+1}{8192}, \hskip 30 pt
k=0,1,2.$$
In particular, Equation ref{reconstruct} holds
for $3$ parameters which are all within $1/1000$
of $1/2$.
\end{lemma}

\startproof
Let $L|_A$ and $R|_A$ denote the
left and right hand sides of
Equation \ref{reconstruct}.
Both $L|_A$ and $R|_A$ are locally affine maps from
an affine lattice into an abelian group.  For
this reason, to check that $L|_A=R|_A$, it suffices to check
the result for $3$ general position points of
$\Theta_A$.  For each choice of $A$ we check this
with a direct computation
for the $4$ lattice points nearest to
$(4\beta_1,4\beta_2)$, where
$\beta_1,\beta_2 \in \{0,1\}$.
\endproof

Define $z_0=(0,0)$ and $z_1=(1,0)$ and $z_2=(0,1)$.
Let $\xi_j=\T_A(z_j) \in \Theta_A$.
The curve $A \to L|_A(\xi_j)$ has an obvious lift $\lambda_j$ to
$\R^2$, namely $\lambda_j(A)=\xi_j$.  The curve
$A \to R_A(\xi_j)$ has a unique lift $\rho_j$ to $\R^2$
such that $\rho_j(1/2)=\lambda_j(1/2)$.
We think of $\lambda_j$ and $\rho_j$ as maps 
from the parameter space into $\R^2$.
Lemma \ref{easy} tells us that
$\lambda_0=\rho_0$.

Inspecting the maps involved, we see that
\begin{equation}
\label{cubic}
\chi(A)=\big(\lambda_j(A)\!-\!\lambda_0(A)\big)\!-\!
\big(\rho_j(A)\!-\!\rho_0(A)\big)=
\left(\frac{\sum_{k=0}^3{a_{jk}A^k}}{(1+A)^3},
\frac{\sum_{k=0}^3{b_{jk}A^k}}{(1+A)^3}\right)
\end{equation}
For certain constants $a_{jk},b_{jk} \in \R$.
Moreover, the curve $A \to \chi(A)$ is (easily)
less than $1000$-Lipschitz on the interval
$[1/2,1/2+1/1000]$.

It follows from Lemma \ref{explicit} that
$\chi(A) \in \Z^2$ for at least $4$ values
of $A$ in the interval $[1/2,1/2+1/1000]$.
The Lipschitz condition then says that
$\chi(A)=(0,0)$ for these $4$ values.
But then each coordinate of
$\chi(A)$ is a rational function of degree $3$.
Such a function cannot have $4$ zeros unless it is
constant.  Hence $\chi(A)$ vanishes identically.
Now we know that
$\lambda_j=\rho_j$ for $j=0,1,2$.   But then
we know that $L|_A(\xi_j)=R|_A(\xi_j)$ for
$j=0,1,2$ and all $A$.  As we mentioned
in the proof of Lemma \ref{explicit}, this suffices
to prove that $L|_A=R|_A$ for all $A$.

\subsection{Images of Vertical Lines}

In this section we will delve more deeply
into how the maps $g_{\pm}$ interact
with the vertical lines. It follows
from the reconstruction formula that
$g_{\pm}(\xi)$ is very close to the
plane $z=0$ when $\xi$ lies close to
a $\cal V$ line.  In this section we will
give more information about this.

\begin{lemma}
\label{particle}
Suppose that $L_1$ and $L_2$ are lines of
$\cal V$ and $L_2=L_1+(\omega,0)$.
Then $g_{\pm}(L_2)=g_{\pm}(L_1)+(\mu,0,0)$, where
$\mu$ is the appropriate representative of
$4p$ mod $1+A$.  In particular, the images
of these lines have the same $y$ and $z$ coordinates.
\end{lemma}

\startproof
It suffices to prove that
$V=(\omega,\omega,\omega) \equiv (4p,0,0)$ mod $\Lambda_A$.
First, we subtract off $\omega$ times the third vector
to get $V \equiv (2\omega,2\omega,0)$ mod
$\Lambda$.  Since $q(1+A)=\omega$, we can subtract off
$2q$ times the second vector and 
get $V \equiv(4p,0,0)$ mod $\Lambda_A$, as desired.
\endproof

The next result gives the first hint of the connection
between the arithmetic graph and the plaid model,
in that it gives some geometric interpretation 
for the capacities.

\begin{lemma}[Vertical Image]
$g_{\pm}$ maps the
$\cal V$ lines of capacity $2k$ and
sign $(\mp)$ into
the segment $$
\big([0,1+A] \times \{\pm k/q\} \times \{0\}\big) \pm (1,1,0).$$
\end{lemma}

\startproof
Given Lemma \ref{particle}, and the locally affine
nature of the maps $g_{\pm}$, it suffices to prove
this result for the lines of capacity $k=1$ which
belong to the first block.  In fact, by symmetry,
it suffices to consider the line $x=x_0$ where
$x_0 \in (0,\omega)$ satisfies
$2px_0 \equiv -1$ mod $\omega$.  
In other words, it suffices to prove that
\begin{equation}
\label{cong1}
(x_0,x_0,x_0) \equiv (t,1/q,0) \hskip 10 pt
{\rm mod\/} \hskip 5 pt \Lambda_A.
\end{equation}
Since $x_0 \in \Z$, we have
$(x_0,x_0,x_0) \equiv (2x_0,2x_0,0)$ mod $\Lambda_A$.
We only have to worry about the second coordinate, so
Equation \ref{cong1} is equivalent to the statement that
\begin{equation}
\label{cong2}
2x_0 = k+kA + \frac{1}{q},
\end{equation}
for some $k \in \Z$.

We know that $2x_0p= k_1\omega -1$.
Since $q=\omega-p$, we have
$2x_0q= k\omega+1$.  Dividing by
$q$ and recalling that $\omega/q=1+A$, we
get Equation \ref{cong2}.
\endproof

\subsection{Images of Horizontal Lines}

If we restrict the classifying map to a horizontal
line, the image is quite dense in $R_A$.
(For irrational parameters, the image is dense.)
To understand how the arithmetic graphs looks
near a horizontal line, we introduce new maps.
The new maps look very different, but they have
the same action on the lattice $\Theta_A$.

Following [{\bf S0\/}, \S 15.3] we introduce maps
$\Delta_{\pm}: \Z^2 \to \R^3$ by the formulas:
$$\Delta_-(m,n)=\Delta_+(m,n)+(-A,A,0), \hskip 30 pt
\Delta_+(m,n)=(x,y,z),$$
\begin{equation}
x=2A(1-m+n)-n, \hskip 12 pt
y=A-x, \hskip 12 pt z=Am.
\end{equation}
Both these maps carry $\Z^2$ into the
plane $x+y=A$.

Recall that $f_{\pm}: \Z^2 \to \R_A$ is the
classifying map from the Master Picture Theorem.
The following result is taken from [{\bf S0\/}]. 
We abbreviate the proof given in
[{\bf S0\/}].

\begin{lemma}
$\Delta_{\pm} = f_{\pm}$ mod $\Lambda_A$.
\end{lemma}

\startproof
Let $v_1,v_2,v_3$ denote the three columns of the
matrix defining $\Lambda_A$.  Let
$$c_1=-1+2m, \hskip 30 pt
1-m+2n, \hskip 30 pt c_3=n.$$
A direct calculation shows that
$$f_{\pm}(m,n)-\Delta_{\pm}(m,n)=c_1v_1+c_2v_2+c_3v_3.$$
\endproof

As with the original classifying map, we pull
these maps back to the lattice
$\Theta_A$ by the formulas
\begin{equation}
h^*_{\pm} = \Delta_{\pm} \circ T_A.
\end{equation}
Since it is a locally affine map,
we can extend $h^*_{\pm}$ to all of
$\R^2$.  The two maps
$h_{\pm}$ have the same action on
$\Theta_A$, at least mod $\Lambda_A$.
However, they act very differently on
$\R^2$. The maps $h^*_{\pm}$ are
not our final maps.  Brlow, we will adjust
these maps by a suitable constant to
get exactly what we want.

Before we do the adjusting, we
describe the main difference
between $h^*_{\pm}$ and $g_{\pm}$.
Let $H$ be a horizontal line.
A straightforward matrix calculation shows
\begin{equation}
\frac{\partial h^*_{\pm}}{\partial x}=
\frac{2p^2}{(p+q)^2} (-A,A,1).
\end{equation}
$h^*_{\pm}(H)$ is parallel to 
$(-A,A,1)$, a vector which lies in
$\Lambda_A$.  Hence, the image of
$h_{\pm}(H)$ in $R_A$ is a closed geodesic
loop. 

Now we adjust $h^*_{\pm}$ so that it is
more useful to us.  Let 
$(\xi \omega,0)$ be the point from
\S \ref{coincidence}.

\begin{lemma}[Horizontal Image]
$h_+^*(\xi \omega,0) \equiv (-1/q,1,0)$ mod $\Lambda_A$.
\end{lemma}

\startproof
Since $(\xi \omega,0) \in \Theta_A$, we have
$$h_+^*(\xi\omega,0)=g_+(\xi \omega,0) =
(\xi\omega,\xi\omega+1,\xi\omega) \hskip 5 pt
{\rm mod\/} \hskip 5 pt \Lambda_A.$$
Since $\xi\omega \in \Z$ and since
$(-1,-1,1) \in \Lambda_A$, we have
$$h^*_{\pm}(\xi \omega,0) =
(2\xi\omega,2\xi\omega+1,0) \hskip 5 pt
{\rm mod\/} \hskip 5 pt \Lambda_A.$$

Subtracting the vector
$2q\xi(1-A,1+A,0) \in \Lambda_A$, we see that
$$h^*(\xi\omega,0) =
(4p\xi,1,0)  \hskip 5 pt
{\rm mod\/} \hskip 5 pt \Lambda_A.$$
So, to finish the proof, we just have
to establish that
$$4\xi p = -1/q \hskip 5 pt
{\rm mod\/} \hskip 5 pt (1+A).$$
Rearranging the terms, we see that this is
equivalent to the existence of some
$K \in \Z$ such that
$4\xi pq+1=K\omega.$
Since $q \equiv -1$ mod $\omega$, this fact follows
from the definition of $\xi$.
\endproof

So, there is some vector $\lambda_A \in \Lambda_A$ such
that 
\begin{equation}
h^*_+(\xi\omega,0)+\lambda_A=(-1/q,1,0).
\end{equation}
We define
\begin{equation}
h_{\pm}=h^*_{\pm} + \lambda_A.
\end{equation}
The map $h_{\pm}$ is just a translated
version of $h^*_{\pm}$.  The two maps
have the same linear part.

\end{document}





















==> Backup/poly.tex <==
\section{Polygon Families}

\subsection{Nice Families}
\label{poly}

In this chapter we prove a result which is similar
in spirit to Lemma \ref{vertical1} but more general.
This result will allow us to compare diverse
families of polygons, such as those shown in
Figure 1.

Let $F$ be a union of pairwise disjoint and
embedded polygons in the plane.  We say that
$F$ {\it sits poorly \/} with respect to a
square $S$ if there is some horizontal line which
 intersects two components of $F \cap S$.
Figure 3.1 shows some examples of this.
Otherwise we say that $F$ {\it sits nicely\/}
with respect to $S$.

\begin{center}
\resizebox{!}{2in}{\includegraphics{Pix/poor.eps}}
\newline
{\bf Figure 3.1:\/} polygons sitting poorly
with respect to squares
\end{center}

We say that $F$ is {\it nice\/} if 
\begin{enumerate}
\item $F$ sits
nicely with respect to every integer unit square.
\item $F$ does not cross an integer vertical line at a
vertex of an integer square.
\item $F$ crosses each unit vertical edge at most once.
\end{enumerate}

There are some situations where $F$ will contain a
point on a unit vertical edge, but not cross there.
We do not count these as intersections. 

A special example comes from the plaid model.
We say that $F$ is {\it standard\/} if,
for every unit integer square,
$F \cap S$ is either the emptyset or a
segment connecting the midpoints of
two of the sides of $S$.  Standard families 
are nice.

\subsection{The Vertical Lemma}

Suppose $A$ is a standard family and $B$ is a nice family.
Given an integer vertical line segment $L$, we 
write $A \cap L \approx B \cap L$ these
sets have the same number of points and if the
order-preserving bijection between the points
moves each point by at most $1$ unit. 
In write $a \sim b$ if the bijection just mentioned
maps $a \in A \cap L$ to $b \in B \cap L$.

Let $y(z)$ denote the $y$-coordinate of $z$.
Let $L_1$ and $L_2$ be two consecutive integer
vertical lines.
We say that a {\it switch\/} is a $4$-tuple
$(a_1,b_1,a_2,b_2)$ such that
\begin{itemize}
\item $a_j \in A \cap L_j$ for $j=1,2$
\item $b_j \in B \cap L_j$ for $j=1,2$.
\item $a_j \sim b_j$ for $j=1,2$.
\item $(y(a_1)-y(a_2)) \times ((y(b_1)-y(b_2))<0$.
\end{itemize}
The last condition says that the the ordering
of the points by height switches.  

Let $X$ be a rectangle whose sides are parallel
to the coordinate axes and whose vertices have
integer coordinates.  Let $X_H$ denote the union
of the top and bottom edge of $X$.  Here is our
main result.


\begin{lemma}[Vertical]
Suppose that \begin{enumerate}
\item $A \cap L \approx B \cap L$
for every maximal 
vertical integer segment $L \subset X$.
\item  $A \cap X_H=B \cap X_H = \emptyset$.
\item $(A,B)$ has no switches.
\end{enumerate}
Then there is a
homeomorphism from $A \cap X$ to $B \cap X$
such that corresponding components are
$\sqrt 2$-quasi-isomorphic.  The homeomorphism
extends the bijections already defined on
the vertical integer segments.
\end{lemma}

The rest of the chapter is devoted to proving the 
Vertical Lemma.  We begin with an easy consideration.
We can write $X=X_1 \cup ... \cup X_k$, where each
$X_j$ is a rectangle which is $1$ unit thick.
It suffices to prove our result for each
rectangle $X_j$ separately, because then
the corresponding homeomorphisms
$h_1,...,h_k$ piece together across the
vertical boundaries to produce one global
homeomorphism.  The quasi-isomorphism
constants do not increase when we do this.
Henceforth we assume that $X$ is one unit wide.

\subsection{Lemmas about Components}

Let $X_1$ and $X_2$ denote the left
and right edges of $X$.  Let
\begin{equation}
A_j=A \cap X_j, \hskip 40 pt
B_j=B \cap X_j.
\end{equation}
For $j=1,2$ we have a bijection from
$A_j$ to $B_j$.  We want to extend
this bijection to a homeomorphism
from $X \cap A$ to $X \cap B$.

There are two kinds of components of
$X \cap A$ and $X \cap B$,
those which have their
endpoints on different sides and those
which do not. We call the first kind
of component a {\it crosser\/} and
the second kind of component a
{\it noncrosser\/}.   The following result
holds for both $A$ and $B$.  The result is
obvious for $A$, so we will state and
prove it for $B$.

Given a point $b_1 \in B_1$, we say that a
point $b_2 \in B_2$ is {\it immediately above\/}
$b_1$ if $y(b_2)\geq y(b_1)$ and there is no
point $b_2' \in B_2$ with $y(b_1) \leq y(b_2')<y(b_2)$.
We make a similar definition for the point
{\it immediately below\/} $b_1$.


\begin{lemma}
A non-crosser connects consecutive points
on a boundary component of $X$.
A crosser connects a point on $B_1$ either to the
point in $B_2$ 
immediately above it or to the point immediately
below it.
\end{lemma}

\startproof
Consider the non-crossing case first.
If this is false, then there are two nested
non-crossers, and a horizontal line in one 
of the squares cuts across both of them.
This contradicts the horizontal line
property.

Now consider the crossing case.
Suppose that $\beta$ is a crosser that connects
$b_1$ to $b_2$ and there is some $b_2'$ with
$y(b_1) \leq y(b_2')<y(b_2)$.  Let $\beta'$
be the component of $X \cap B$ which has 
$b_2'$ as an endpoint.  Then the horizontal
line segment through $b_2'$ intersects both
$\beta$ and $\beta'$, contradicting
the horizontal line property.
\endproof

\begin{lemma}
The Vertical Lemma is true provided that
the bijection on the boundary extends to
the crossers.
\end{lemma}

\startproof
Suppose we have a
bijection between the crossers of $A$ and
the crossers of $B$ which extends the
bijection on the boundary.  Then the
consecutive points property guarantees that
the non-crossers form the same pattern
for both $A$ and $B$. This allows us to
extend the bijection to the non-crossers.

It just remains to show that corresponding
components are $\sqrt 2$-quasi-isomorphic.
Let $\alpha$ and $\beta$ be two corresponding
components.  The corresponding endpoints of these
components differ from each other by at
most $1$ unit.  The basic property these paths
have is that once they enter a square from the bottom
they cannot exit the square until they reach
the top.  This follows from the niceness property.
So, $\alpha$ and $\beta$ occupy exactly the
same squares, except possibly at the top at
the bottom, and traverse them in the same
order.  From here it is easy to see that
the curves are $\sqrt 2$-quasi-isomorphic.
Here $\sqrt 2$ is the diameter of a unit
square.
\endproof

\subsection{Extending to the Crossers}

Now we will show that our bijection extends to the
crossers.   We label the points of $A_1$ as
$a_{1,1},...,a_{1,N}$, starting from the bottom.
We label the points of the sets $A_2,B_1,B_2$
similarly.  In general, we say that one point
lies above another if it has a larger $y$-coordinate.
Similarly, a point lies above an interval if
the point lies above the top endpoint of the
interval.

Suppose that we have an $A$-crosser $\alpha$
that connects $a_{1,m}$ to $a_{2,n}$.  We want
to see that there is a $B$-crosser that
connects $b_{1,m}$ to $b_{2,n}$.   Let
$\beta$ be the component of $X \cap B$ which
contains $b_{1,m}$.

\subsubsection{Case 1}

In this subsection we will consider 
the case when $\beta$ is a crosser.
Suppose first that $\alpha$ is not
a horizontal segment.  Then there
Then there is no point of $A_2$ directly
across from $a_{1,m}$.  That means
we have one of two situations.
\begin{itemize}
\item $a_{2,n-1}$ is directly below
$a_{1,m}$ and $a_{2,n}$ is directly above.
\item $a_{2,n}$ is directly below
$a_{1,m}$ and $a_{2,n+1}$ is directly above.
\end{itemize}
In either case, the fact that there are no switches
implies that one of two situations holds:
\begin{itemize}
\item $b_{2,n-1}$ is directly below
$b_{1,m}$ and $b_{2,n}$ is directly above.
\item $b_{2,n}$ is directly below
$b_{1,m}$ and $b_{2,n+1}$ is directly above.
\end{itemize}
But that means that $\beta$ connects
$b_{2,m}$ to one of the three points
$b_k$ for $k \in \{n-1,n,n+1\}$.
Parity considerations rule out two of the
possibilities.  If $\beta$ connects
$b_{1,m}$ to $b_{2,n \pm 1}$ then 
$\beta$ divides the remaining points
of $B_1 \cup B_2$ into two halves, each
containing an odd number of points. But then
these points cannot be paired up by the
arcs of $X \cap B$.  So,
$\beta$ connects $b_{1,m}$ to $b_{2,n}$.

Suppose that $\alpha$ is a
horizontal segment.  In this case,
$A_{1,m}$ and $A_{2,n}$ are directly
across from each other.  If $b_{2,k}$ is
immediately above $b_{1,m}$ for $k \geq n+2$,
then $b_{1,n+1}$ is below $b_{1,m}$ and
we have a switch. So, $b_{2,k}$ cannot
be immediately above $b_{1,m}$ for
$k \geq n+2$.  The same argument shows that
$b_{2,k}$ cannot be immediately below
$b_{1,m}$ for $k \leq n-2$.  From this
we see that $\beta$ can only connect
$b_{1,m}$ to $b_{2,k}$ for
$k \in \{n-1,n,n+1\}$.  The same parity
argument as in the previous case
shows that $\beta$ connects
$b_{1,m}$ to $b_{2,n}$ as desired.
\newline
\newline
{\bf Remark:\/} In both cases, the analysis shows
that the only points which can lie immediately
above $b_{1,m}$ are $b_{2,n}$ and $b_{n+1}$,
and the only points which can lie immediately
below $b_{1,m}$ are $b_{2,n-1}$ nad
$b_{2,n}$.

\subsubsection{Case 2}

Now suppose that $\beta$ is a non-crosser.
Then $\beta$ connects $b_{1,m}$ to $b_{1,m\pm 1}$.
Without loss of generality, consider the case when
$\beta$ connects $b_{1,m}$ to $b_{1,m+1}$.
We claim that $b_{2,n}$ lies above $b_{1,m+1}$.
Since there are no switches, $a_{2,n}$ lies
above $a_{1,m+1}$ or at the same level.
Given the nature of the family $A$, there
can be no points of $A_1$ lying between the
two endpoints of $\alpha$.  This is a contradiction.

Now we deal with our claim.
Since $A$ is a nice family, there are
no points of $B_2$ lying between
$b_{1,m}$ and $b_{1,m+1}$.
The analysis in Case 1 shows that
the only points lying immediately
above $b_{1,m}$ are
$b_{2,n}$ and $b_{2,n+1}$.  In either
case, $b_{2,n+1}$ lies above $b_{1,m}$.
Hence $b_{2,n+1}$ iies above $b_{1,m+1}$.
Similarly, $b_{2,n-1}$ lies below
$b_{1,m}$.

Let $A_1^k$ denote the points of $A_1$ above 
or equal to $a_{1,k}$.
Likewise define $A_{2,k}$, etc.
The points of
$A_1^{m+1} \cup A_2^{n+1}$ have to be paired up with
other components of $X \cap A$.  Hence, this
set has an even number $E$ of points.
Note that $B_1^{m+1} \cup B_2^{n+1}$ has $E$ points
as well.

Since $B$ is a nice family, the
points of $B_1 \cup B_2$ lying above
$b_{1,m+1}$ must be paired together by
the components of $B \cap X$.  
If $b_{2,n}$ lies below $b_{2,m}$, 
then $B_1^{m+2} \cup B_2^{n+1}$ has an
even number of points.  But this is false,
because $B_1^{m+2} \cup B_2^{n+1}$ has $E-1$ points.
This establishes the claim.

\newpage
